Understanding the behavior of the Sun's large scale magnetic field and its relation with the meridional flow

In this thesis, various studies are performed leading to better understanding of the 11-year solar cycle and its theoretical modeling with the flux transport dynamo model. Although this is primarily a theoretical thesis, there is a part dealing with the analysis of observational data. The various proxies of solar activity from various observatory including the sunspot area records of Kodaikanal Observatory have been analyzed to study the irregular aspects of solar cycles and an analysis has been carried out on the correlation between the decay rate and the next cycle amplitude. Theoretical analysis starts with explaining how the magnetic buoyancy has been treated in the flux transport dynamo models, and advantages and disadvantages of different treatments. It is found that some of the irregular properties of the solar cycle in the decaying phase can only be well explained using a particular treatment of the magnetic buoyancy. Next, the behavior of the dynamo with different spatial structures of the meridional flow based on recent helioseismology results has been studied. A theoretical model is constructed considering the back reaction due to the Lorentz force on the meridional flows which explains the observed variation of the meridional flow with the solar cycle. Finally, some results with 3D FTD models are presented. This 3D model is developed to handle the Babcock-Leighton mechanism and magnetic buoyancy more realistically than previous 2D models and can capture some important effects connected with the subduction of the magnetic field in polar regions, which are missed in 2D surface flux transport models. This 3D model is further used to study the evolution of the magnetic fields due to a turbulent non-axisymmetric velocity field and to compare the results with the results obtained by using a simple turbulent diffusivity coefficient.

==> preamble.tex <==
% ******************************************************************************
% ****************************** Custom Margin *********************************

% Add `custommargin' in the document class options to use this section
% Set {innerside margin / outerside margin / topmargin / bottom margin}  and
% other page dimensions
\ifsetCustomMargin
  \RequirePackage[left=37mm,right=30mm,top=35mm,bottom=30mm]{geometry}
  \setFancyHdr % To apply fancy header after geometry package is loaded
\fi

% *****************************************************************************
% ******************* Fonts (like different typewriter fonts etc.)*************

% Add `customfont' in the document class option to use this section

\ifsetCustomFont
  % Set your custom font here and use `customfont' in options. Leave empty to
  % load computer modern font (default LaTeX font).
  \RequirePackage{helvet}
\fi

% *****************************************************************************
% **************************** Custom Packages ********************************

% ************************* Algorithms and Pseudocode **************************

%\usepackage{algpseudocode}


% ********************Captions and Hyperreferencing / URL **********************

% Captions: This makes captions of figures use a boldfaced small font.
%\RequirePackage[small,bf]{caption}

\RequirePackage[labelsep=space,tableposition=top]{caption}
\renewcommand{\figurename}{Fig.} %to support older versions of captions.sty


% *************************** Graphics and figures *****************************

%\usepackage{rotating}
%\usepackage{wrapfig}

% Uncomment the following two lines to force Latex to place the figure.
% Use [H] when including graphics. Note 'H' instead of 'h'
%\usepackage{float}
%\restylefloat{figure}

% Subcaption package is also available in the sty folder you can use that by
% uncommenting the following line
% This is for people stuck with older versions of texlive
%\usepackage{sty/caption/subcaption}
\usepackage{subcaption}

% ********************************** Tables ************************************
\usepackage{booktabs} % For professional looking tables
\usepackage{multirow}

%\usepackage{multicol}
%\usepackage{longtable}
%\usepackage{tabularx}


% ***************************** Math and SI Units ******************************

\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{siunitx} % use this package module for SI units
\usepackage{caption}
\captionsetup{margin=10pt,font=small,labelfont=bf}
\usepackage{deluxetable}
% ******************************* Line Spacing *********************************

% Choose linespacing as appropriate. Default is one-half line spacing as per the
% University guidelines

% \doublespacing
% \onehalfspacing
% \singlespacing


% ************************ Formatting / Footnote *******************************

% Don't break enumeration (etc.) across pages in an ugly manner (default 10000)
%\clubpenalty=500
%\widowpenalty=500

%\usepackage[perpage]{footmisc} %Range of footnote options


% *****************************************************************************
% *************************** Bibliography  and References ********************

%\usepackage{cleveref} %Referencing without need to explicitly state fig /table

% Add `custombib' in the document class option to use this section
\ifuseCustomBib
   \RequirePackage[square, sort, numbers, authoryear]{natbib} % CustomBib

% If you would like to use biblatex for your reference management, as opposed to the default `natbibpackage` pass the option `custombib` in the document class. Comment out the previous line to make sure you don't load the natbib package. Uncomment the following lines and specify the location of references.bib file

%\RequirePackage[backend=biber, style=numeric-comp, citestyle=numeric, sorting=nty, natbib=true]{biblatex}
%\bibliography{References/references} %Location of references.bib only for biblatex

\fi

% changes the default name `Bibliography` -> `References'
\renewcommand{\bibname}{References}


% *****************************************************************************
% *************** Changing the Visual Style of Chapter Headings ***************
% This section on visual style is from https://github.com/cambridge/thesis

% Uncomment the section below. Requires titlesec package.

%\RequirePackage{titlesec}
%\newcommand{\PreContentTitleFormat}{\titleformat{\chapter}[display]{\scshape\Large}
%{\Large\filleft{\chaptertitlename} \Huge\thechapter}
%{1ex}{}
%[\vspace{1ex}\titlerule]}
%\newcommand{\ContentTitleFormat}{\titleformat{\chapter}[display]{\scshape\huge}
%{\Large\filleft{\chaptertitlename} \Huge\thechapter}{1ex}
%{\titlerule\vspace{1ex}\filright}
%[\vspace{1ex}\titlerule]}
%\newcommand{\PostContentTitleFormat}{\PreContentTitleFormat}
%\PreContentTitleFormat


% ******************************************************************************
% ************************* User Defined Commands ******************************
% ******************************************************************************

% *********** To change the name of Table of Contents / LOF and LOT ************

%\renewcommand{\contentsname}{My Table of Contents}
%\renewcommand{\listfigurename}{My List of Figures}
%\renewcommand{\listtablename}{My List of Tables}


% ********************** TOC depth and numbering depth *************************

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}


% ******************************* Nomenclature *********************************

% To change the name of the Nomenclature section, uncomment the following line

%\renewcommand{\nomname}{Symbols}


% ********************************* Appendix ***********************************

% The default value of both \appendixtocname and \appendixpagename is `Appendices'. These names can all be changed via:

%\renewcommand{\appendixtocname}{List of appendices}
%\renewcommand{\appendixname}{Appndx}

% ******************************** Draft Mode **********************************

% Uncomment to disable figures in `draftmode'
%\setkeys{Gin}{draft=true}  % set draft to false to enable figures in `draft'

% These options are active only during the draft mode
% Default text is "Draft"
%\SetDraftText{DRAFT}

% Default Watermark location is top. Location (top/bottom)
%\SetDraftWMPosition{bottom}

% Draft Version - default is v1.0
%\SetDraftVersion{v1.1}

% Draft Text grayscale value (should be between 0-black and 1-white)
% Default value is 0.75
%\SetDraftGrayScale{0.8}


%% Todo notes functionality
%% Uncomment the following lines to have todonotes.

%\ifsetDraft
%	\usepackage[colorinlistoftodos]{todonotes}
%	\newcommand{\mynote}[1]{\todo[author=kks32,size=\small,inline,color=green!40]{#1}}
%\else
%	\newcommand{\mynote}[1]{}
%	\newcommand{\listoftodos}{}
%\fi

% Example todo: \mynote{Hey! I have a note}




==> thesis-info.tex <==
\nonstopmode % Do not stop if the font is not available
% boldface
\newfont{\degfntbf}{eufb10 scaled\magstep3} 
% Bigger
\newfont{\degfnt}{eufm10 scaled\magstep3} 
\errorstopmode % revert back to stop on error
\nonstopmode % Do not stop if the font is not available
\newfont{\titlefnt}{cmssdc10 scaled\magstep3} 
\newfont{\Titlefnt}{cmssdc10 scaled\magstep4} 
\newfont{\twelvessf}{lcmss8 scaled\magstep2}
\errorstopmode % revert back to stop on error

% These macros define an environment for front matter that is always 
% single column even in a double-column document.
\newenvironment{alwayssingle}{%
       \@restonecolfalse\if@twocolumn\@restonecoltrue\onecolumn
       \else\newpage\fi}
       {\if@restonecol\twocolumn\else\newpage\fi}


% \author, \title are defined in report; here are the rest of the
% front matter defining macros
\def\dept#1{\gdef\@dept{#1}}
%\def\enggfaculty{\gdef\@faculty{Faculty of Engineering}}
\def\sciencefaculty{\gdef\@faculty{Faculty of Science}}
\def\degreein#1{\gdef\@faculty{#1}}
\def\submitdate#1{\gdef\@submitdate{#1}}
\def\degree#1{\gdef\@degree{#1}}
\def\phd{\gdef\@degree{Doctor of Philosophy}}
\def\mscengg{\gdef\@degree{Master of Science (Engineering)}}
\def\me{\gdef\@degree{Master of Engineering}\metrue}
\def\bibtitle#1{\gdef\@bibtitle{#1}}
\def\faculty#1{\gdef\@faculty{#1}}

\newif\iffigurespage \newif\iftablespage 
\newif\ifiisclogo 
\newif\ifme % To print project report in the title page

\figurespagetrue \tablespagefalse 
\iisclogofalse \mefalse
\def\iisclogo#1{
	% For first  call,   load the  file  iisclogo.sty  which  will
	% redefine this macro!
	\makeatletter\input{iisclogo.sty}\makeatother
	\iisclogo{#1}
	}

% From titlepage.sty  27 Jan 85
\renewcommand{\maketitle}{%
\begin{titlepage}\begin{singlespace}
\setcounter{page}{0}
%\null
\vskip -1.0in
	%{\baselineskip 1cm
	{\huge %\baselinestretch{4}
	\begin{center}
		%\Huge\uppercase\expandafter{\@title} 
		{\Titlefnt \@title} 
	\end{center} \par} % The spacing between second and  third line
			   % is not proper
\vfill
\begin{center}
	%\sc 
	\Large \twelvessf 
	A \ifme Project Report \else Thesis \fi \\
	Submitted \ifme in partial fulfilment of the \\
	requirements for \else for \fi the Degree of\\
	{\degfntbf \@degree} \\
	%\sc
	\Large \twelvessf 
	in \ifme \\ \else the \fi {\degfntbf \@faculty }
\end{center}
\vfill
	{\lineskip .75em
	\begin{center}
	\twelvessf 
	by \\[0.75em]
	{\large \bf \@author}
	\end{center}\par} 
\vfill

	\vfill
	\begin{center}
	\begin{figure}[h!]
	  \centering
	  \includegraphics[height=1.5in]{IISc1.eps}
 % IISc1.png: 526x488 pixel, 72dpi, 18.56x17.22 cm, bb=
	\end{figure}
%	\iisclogo{950} % Laser printer gives error 21 for lower sizes
	\end{center}

\vfill
\begin{center}
 	\large \twelvessf 
	\@dept \\
 	Indian Institute of Science \\
 	Bangalore -- 560 012 (INDIA)\\[0.75em]
	\@submitdate\\
\end{center}
\vskip -0.5in
\null
\end{singlespace}\end{titlepage}
%\pagenumbering{roman} % Already in frotmater env!
} %maketitle




